A Stochastic Decoupling Method for Minimizing the Sum of Smooth and Non-Smooth Functions

We consider the problem of minimizing the sum of three convex functions: i) a smooth function $f$ in the form of an expectation or a finite average, ii) a non-smooth function $g$ in the form of a finite average of proximable functions $g_j$, and iii) a proximable regularizer $R$. We design a variance-reduced method which is able to progressively learn the proximal operator of $g$ via the computation of the proximal operator of a single randomly selected function $g_j$ in each iteration only. Our method can provably and efficiently accommodate many strategies for the estimation of the gradient of $f$, including via standard and variance-reduced stochastic estimation, effectively decoupling the smooth part of the problem from the non-smooth part. We prove a number of iteration complexity results, including a general ${\cal O}(1/t)$ rate, ${\cal O}(1/t^2)$ rate in the case of strongly convex smooth $f$, and several linear rates in special cases, including accelerated linear rate. For example, our method achieves a linear rate for the problem of minimizing a strongly convex function $f$ subject to linear constraints under no assumption on the constraints beyond consistency. When combined with SGD or SAGA estimators for the gradient of $f$, this leads to a very efficient method for empirical risk minimization. Our method generalizes several existing algorithms, including forward-backward splitting, Douglas-Rachford splitting, proximal SGD, proximal SAGA, SDCA, randomized Kaczmarz and Point-SAGA. However, our method leads to many new specific methods in special cases; for instance, we obtain the first randomized variant of the Dykstra's method for projection onto the intersection of closed convex sets.

==> algs/double_alg_minibatch.tex <==
\begin{algorithm}[t]
   \caption{Double method with minibatching.}
   \label{alg:double_mini}
\begin{algorithmic}[1]
   \Require Stepsize $\eta$, initial vectors $x^0$, $y_1^0, \dotsc, y_m^0$, oracle that gives gradient estimates
   \For{$t=0,1,\dotsc$}
	   \State Produce a gradient estimate $v^t$, and set $y^t = \avekm y_k^t$
	   \State $z^{t} = \proxR(x^t - \eta v^t - \eta y^t)$
	   \State Sample $S$ such that $|S|=b$, $\Pb(j\in S)=p_j$ and set $\eta_j = \frac{\eta}{mp_j}$
	   \For{$j\in S$}
		   \State $x_j^{t+1} = \proxj(z^t + \eta_j y_j^t)$
		   \State $y_j^{t+1} = y_j^t + \frac{1}{\eta_j}(z^t - x^{t+1})$
	   \EndFor
	   \State $x^{t+1} = \frac{1}{b}\sum_{j\in S}x_j^{t+1}$
   \EndFor
\end{algorithmic}
\end{algorithm}

==> algs/gd.tex <==
\begin{algorithm}[!h]
   \caption{Stochastic Decoupling Method with Gradient Descent.}
   \label{alg:sdm_gd}
\begin{algorithmic}[1]
   \Require Stepsize $\eta$, initial vectors $x^0$, $x^0$, $y_1^0, \dotsc, y_m^0\in \RR^d$, $y^0=\avejm y_j^0$, probabilities $p_1,\dotsc, p_m$
   \For{$t=0,1,\dotsc$}
	   \State $z^{t+1} = \proxR(x^t - \eta \nabla f(x^t) - \eta y^t)$
	   \State Sample $j$ from $\{1,\dotsc, m\}$ with probabilities $\{p_1, \dotsc, p_m\}$ and set $\eta_j = \frac{\eta}{mp_j}$
	   \State $x^{t+1} = \proxj(z^t + \eta_j y_j^t)$
	   \State $y_j^{t+1} = y_j^t + \frac{1}{\eta_j}(z^t - x^{t+1})$
	   \State $y^{t+1} =  y^t + \frac{1}{m}(y_j^{t+1} - y_j^t)$
   \EndFor
\end{algorithmic}
\end{algorithm}

==> algs/katyusha.tex <==
\begin{algorithm}[t]
   \caption{Double-VR with Katyusha.}
   \label{alg:double_kat}
\begin{algorithmic}[1]
   \Require Parameter $\theta_1$, $\theta_2=\frac{1}{2}$, initial vectors $x^0$, $y_1^0, \dotsc, y_m^0$, $y^0=\avejm y_j^0$
   \For{$t=0,1,\dotsc$}
       \State $m^t = \theta_1 x^t + \theta_2 u^t + \left(1 - \theta_1 - \theta_2\right)h^t$
       \State Sample $i$ uniformly from $\{1, \dotsc, n\}$
	   \State $v^t = \nabla f_i(m^t) - \nabla f_i(u^t) + \nabla f(u^t)$
	   \State $z^{t} = \proxR(x^t - \eta v^t - \eta y^t)$
	   \State Sample $j$ from $\{1,\dotsc, m\}$ with probabilities $\{p_1, \dotsc, p_m\}$ and set $\eta_j = \frac{\eta}{mp_j}$
	   %\State $w^{t+1} = z^{t+1} - \eta(y_j^t - y^t)$
	   %\State $u^{t} = \proxj(w^{t+1}) - x^{t+1}$
	   \State $x^{t+1} = \proxj\left(z^t + \eta_j y_j^t\right)$
	   \State $y_j^{t+1} = y_j^t + \frac{1}{\eta_j}(z^{t} - x^{t+1})$
	   \State $ y^{t+1} =  y^t + \frac{1}{m}(y_j^{t+1} - y_j^t)$
	   \State $h^{t+1} = m^t + \theta_1(x^{t+1} - x^t)$
	   \State $u^{t+1} = \begin{cases} h^{t+1}, & \text{with probability } \frac{1}{n}, \\ u^t, & \text{with probability } 1 - \frac{1}{n} \end{cases}$
   \EndFor
\end{algorithmic}
\end{algorithm}

==> algs/saga.tex <==
\begin{algorithm}[!h]
   \caption{Stochastic Decoupling Method with SAGA.}
   \label{alg:sdm_saga}
\begin{algorithmic}[1]
   \Require Stepsize $\eta$, initial vectors $x^0$, $\nabla f_1(u_1^0), \dotsc, \nabla f_n(u_n^0)$, $\alpha^0=\avein \nabla f_i(u_i^0)$, $y_1^0, \dotsc, y_m^0$, $y^0=\avejm y_j^0$, minibatch size $\tau$, probabilities $p_1,\dotsc, p_m$, $q_1,\dotsc, q_n$
   \For{$t=0,1,\dotsc$}
	   \State Sample subset $S$ from $\{1,\dotsc, n\}$ of size $\tau$ with probabilities $q_1, \dotsc, q_n$
	   \State $v^t= \sum_{i\in S}\frac{1}{q_i n}\left(\nabla f_i(x^t) - \nabla f_i(u_i^t)\right) + \alpha^t$
	   \State $z^{t} = \proxR(x^t - \eta v^t - \eta y^t)$
	   \For{$i\in S$}
	   	\State Update $\nabla f_i(u_i^{t+1})$ with $u_i^{t+1} = x^t$
	   \EndFor
	   \State $\alpha^{t+1} = \alpha^t + \frac{1}{n}\sum_{i\in S}(\nabla f_i(u_i^{t+1}) - \nabla f_i(u_i^t))$
	   \State Sample $j$ from $\{1,\dotsc, m\}$ with probabilities $\{p_1, \dotsc, p_m\}$ and set $\eta_j = \frac{\eta}{mp_j}$
	   %\State $w^{t+1} = z^{t+1} - \eta(y_j^t - y^t)$
	   %\State $u^{t} = \proxj(w^{t+1}) - x^{t+1}$
	   \State $x^{t+1} = \proxj\left(z^t + \eta_j y_j^t\right)$
	   \State $y_j^{t+1} = y_j^t + \frac{1}{\eta_j}(z^{t} - x^{t+1})$
	   \State $ y^{t+1} =  y^t + \frac{1}{m}(y_j^{t+1} - y_j^t)$
   \EndFor
\end{algorithmic}
\end{algorithm}

==> algs/sgd.tex <==
\begin{algorithm}[t]
   \caption{Double with SGD.}
   \label{alg:double_sgd_saga}
\begin{algorithmic}[1]
   \Require Stepsize $\eta$, initial vectors $x^0$, $y_1^0, \dotsc, y_m^0$, $y^0=\avejm y_j^0$, oracle that unbiased gradient estimates
   \For{$t=0,1,\dotsc$}
	   \State $z^{t+1} = x^t - \eta \nabla f(x^t; \xi)$
	   \State Sample $j$ from $\{1,\dotsc, m\}$ with probabilities $\{p_1, \dotsc, p_m\}$ and set $\eta_j = \frac{\eta}{mp_j}$
	   \State $w^{t+1} = z^{t+1} - \eta(y_j^t - y^t)$
	   \State $u^{t} = \proxj(w^{t+1}) - x^{t+1}$
	   \State $y_j^{t+1} = \frac{1}{\eta}(x^{t+1} - w^{t+1})$
	   \State $ y^{t+1} =  y^t + \frac{1}{m}(y_j^{t+1} - y_j^t)$
   \EndFor
\end{algorithmic}
\end{algorithm}

==> algs/v_gd.tex <==
\begin{algorithm}[t]
   \caption{Gradient Descent Oracle.}
   \label{alg:v_gd}
\begin{algorithmic}[1]
	\Require $x^t$\\
	\Return $v^t=\nabla f(x^t)$
\end{algorithmic}
\end{algorithm}
